Drift-free Visual SLAM using Digital Twins

Globally-consistent localization in urban environments is crucial for autonomous systems such as self-driving vehicles and drones, as well as assistive technologies for visually impaired people. Traditional Visual-Inertial Odometry (VIO) and Visual Simultaneous Localization and Mapping (VSLAM) methods, though adequate for local pose estimation, suffer from drift in the long term due to reliance on local sensor data. While GPS counteracts this drift, it is unavailable indoors and often unreliable in urban areas. An alternative is to localize the camera to an existing 3D map using visual-feature matching. This can provide centimeter-level accurate localization but is limited by the visual similarities between the current view and the map. This paper introduces a novel approach that achieves accurate and globally-consistent localization by aligning the sparse 3D point cloud generated by the VIO/VSLAM system to a digital twin using point-to-plane matching; no visual data association is needed. The proposed method provides a 6-DoF global measurement tightly integrated into the VIO/VSLAM system. Experiments run on a high-fidelity GPS simulator and real-world data collected from a drone demonstrate that our approach outperforms state-of-the-art VIO-GPS systems and offers superior robustness against viewpoint changes compared to the state-of-the-art Visual SLAM systems.

==> figures/factorGraph.tex <==
%!TEX root=Plots.tex
\tikzstyle{every node}=[font=\footnotesize]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\begin{tikzpicture}[>=stealth]
\def\l{0.2cm}
\def\r{0.25cm}
\def\w{0.5cm}
\def\h{\w}

\def\ws{0.3cm}
\def\hs{\ws}

\tikzstyle{factor}=[
	fill = matlab1,
	fill opacity = 1,
	draw = matlab1,
	draw opacity = 1,
	text opacity = 1,
	minimum width = \w,
	minimum height = \h,
	anchor = center,
	inner sep = 0pt,
	outer sep = 0pt,
	]
	

\tikzstyle{landmark}=[
	fill = matlab1!10!white,
	fill opacity = 1.0,
	draw = matlab1!50!white,
	draw opacity = 1,
	text opacity = 1,
	star,
	star points = 7,
	star point ratio=0.4,
	minimum width = 0.7*\l,
	minimum height = 0.7*\l,
	anchor = center,
	inner sep = 0pt,
	outer sep = 0pt,
	]
	
\tikzstyle{robot}=[
	fill = black,
	fill opacity = 0.75,
	draw = black,
	draw opacity = 1,
	text opacity = 1,
	circle,
	minimum width = \r,
	minimum height = \r,
	anchor = center,
	inner sep = 0pt,
	outer sep = 0pt,
	]

\tikzstyle{point3D}=[
	fill = matlab1!20!white,
	fill opacity = 0.75,
	draw = matlab1,
	draw opacity = 1,
	text opacity = 1,
	circle,
	minimum width = \r,
	minimum height = \r,
	anchor = center,
	inner sep = 0pt,
	outer sep = 0pt,
	]

\tikzstyle{vision factor}=[
	factor,
	fill = matlab1!20!white,
	draw = matlab1,
	]

\tikzstyle{inertial factor}=[
	factor,
	fill = matlab2!20!white,
	draw = matlab2,
	]
	
\tikzstyle{map factor}=[
	factor,
	fill = matlab4!20!white,
	draw = matlab4,
	]
	
\tikzstyle{initial factor}=[
	factor,
	fill = matlab3!20!white,
	draw = matlab3,
	]
		

\tikzstyle{see inertial}=[
	color=matlab2,
	]
	
\tikzstyle{see map}=[
	color=matlab4,
	]

\tikzstyle{see landmark}=[
	color=matlab1,
	]

\tikzstyle{see robot}=[
	color=black,
	]
	

\node [vision factor, rotate=-15] at (1,3) (v1) {V};
\node [vision factor, rotate=0] at (3,3.5) (v2) {V};
\node [vision factor, rotate=5] at (5,3) (v3) {V};
\path (v1) -- coordinate[pos=0.5] (v12) (v2);
\path (v2) -- coordinate[pos=0.5] (v23) (v3);

\node [inertial factor, rotate=8] at ( v12 |- 0,2.8 ) (i1) {I};
\node [inertial factor, rotate=-5] at ( v23 |- 0,2.9 ) (i2) {I};

\begin{pgfonlayer}{foreground}
\node [robot] at (1, 2.3) (r1) {};
\node [robot] at (3, 2.3) (r2) {};
\node [robot] at (5, 2.3) (r3) {};
\end{pgfonlayer}

\node [map factor, below = 15mm of v23, text width = 20mm, inner sep = 3pt, align=center, minimum width = 30mm] (map) {Geometric Digital Twin};
\draw [see map] (r1) -- (map.north west);
\draw [see map] (r2) -- (map.north -| r2);
\draw [see map] (r3) -- (map.north -| r3);

\node [initial factor, below = 5mm of r1, text width = 10mm, inner sep = 3pt, align=center] (init) {Initial GPS};
\draw [color=matlab3] (init) -- (r1);

\node [point3D] at (0.5,4.5) (l1) {};
\node [point3D] at (1.3,4.4) (l2) {};
\node [point3D] at (2.7,4.7) (l3) {};
\node [point3D] at (3.8,4.6) (l4) {};
\node [point3D] at (4.3,4.4) (l5) {};
\node [point3D] at (5.4,4.5) (l6) {};

\draw [see landmark] (v1.north) -- (l1);
\draw [see landmark] (v1.north) -- (l2);
\draw [see landmark] (v2.north) -- (l2);
\draw [see landmark] (v2.north) -- (l3);
\draw [see landmark] (v2.north) -- (l4);
\draw [see landmark] (v2.north) -- (l5);
\draw [see landmark] (v3.north) -- (l4);
\draw [see landmark] (v3.north) -- (l5);
\draw [see landmark] (v3.north) -- (l6);

\draw [see inertial] (r1) -- (i1);
\draw [see inertial] (i1) -- (r2);
\draw [see inertial] (r2) -- (i2);
\draw [see inertial] (i2) -- (r3);

\draw [see robot] (r1) -- (v1);
\draw [see robot] (r2) -- (v2);
\draw [see robot] (r3) -- (v3);

\node at ([xshift=0.7cm]l6 |- v3) (tab1) {};
\node at ([xshift=0.9cm]l6 |- v3) (tab2) {};


\node [anchor = west, align=left, text width = 2cm] at ([yshift=0mm]tab2) (i) {Inertial Factor};
\node [anchor = west, align=left, text width = 2cm, above = 0mm of i] (v) {Vision Factor};
\node [anchor = west, align=left, text width = 2cm, above = 0mm of v] (l) {Vision Landmark};
\node [anchor = west, align=left, text width = 2cm, above = 0mm of l] (q) {Camera State};

\node [inertial factor, minimum width = 0.25cm, minimum height = 0.25cm] at (tab1 |- i) {I};
\node [vision factor, minimum width = 0.25cm, minimum height = 0.25cm] at (tab1 |- v) {V};
\node [point3D] at (tab1 |- l) {};
\node [robot, minimum width = 0.25cm, minimum height = 0.25cm] at (tab1 |- q) {};

\end{tikzpicture}%

==> figures/figureGPS/figure_gps.tex <==
\begin{tikzpicture}[>=latex]
\tikzstyle{every node}=[font=\footnotesize]

\tikzstyle{groundtruth}=[black, thick,  line join=bevel]
\tikzstyle{methods}=[thick, line join=bevel]

\begin{axis} [
	at={(0cm, 0cm)},
	width = 7.5cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {y [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 2,
     legend cell align={left},
     legend style ={
     	at = {(0.5, 1.04)},
         draw = none,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
         anchor=south,
         name=legend,
     },
%     xmin=-20.0,
%     xmax=120.0,
%     ymin=-10.0,
%     ymax=160.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot1,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=y, col sep=space, ignore chars={\#}] {figures/figureGPS/stamped_groundtruth.txt};

\addplot+ [methods, only marks, mark options={scale=0.5}] table [x=x, y=y, col sep=space, ignore chars={\#}, each nth point=3, filter discard warning=false, unbounded coords=discard ] {figures/figureGPS/gps.txt};

\addlegendentry{Groundtruth};
\addlegendentry{GPS};
\end{axis}

\begin{axis} [
	at={(0cm, -5cm)},
	width = 7.5cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {z [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 1,
     legend cell align={left},
     legend style ={
         draw = gray,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
     },
%     xmin=-10.0,
%     xmax=120.0,
%     ymin=-5,
%     ymax=30.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot2,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=z, col sep=space, ignore chars={\#}] {figures/figureGPS/stamped_groundtruth.txt};

\addplot+ [methods, only marks, mark options={scale=0.5}] table [x=x, y=z, col sep=space, ignore chars={\#}, each nth point=3, filter discard warning=false, unbounded coords=discard ] {figures/figureGPS/gps.txt};

\end{axis}

\draw (legend.north -| plot1.west) rectangle (legend.south -| plot1.east);

\end{tikzpicture}

==> figures/figureRealworld/figure_realworld.tex <==
%!TEX root = ../Plots.tex

\begin{tikzpicture}[>=latex]
\tikzstyle{every node}=[font=\footnotesize]

\tikzstyle{groundtruth}=[black, thick,  line join=bevel]
\tikzstyle{methods}=[thick, line join=bevel]

\begin{axis} [
	at={(0cm, 0cm)},
	width = 7.7cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {y [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 6,
     legend cell align={left},
     legend style ={
     	at = {(1.0, 1.04)},
         draw = none,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
         anchor=south,
         name=legend,
     },
%     xmin=-20.0,
%     xmax=120.0,
%     ymin=-10.0,
%     ymax=160.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot1,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=y, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard] {figures/figureRealworld/VINS/stamped_groundtruth.txt};

\foreach \f in {VINS,SVO_GPS, SVO_LC,ORB,SVO-MR} {
	\addplot+ [methods] table [x=x, y=y, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard ] {figures/figureRealworld/\f/stamped_traj_estimate_aligned.txt};
}

\addlegendentry{Groundtruth};
\addlegendentry{VINS-Fusion};
\addlegendentry{SVO-GPS};
\addlegendentry{SVO-Loop Closure};
\addlegendentry{ORB-SLAM3};
\addlegendentry{SVO-Digital Twin (ours)};
\end{axis}

\begin{axis} [
	at={(8.5cm, 0cm)},
	width = 7.5cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {z [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 1,
     legend cell align={left},
     legend style ={
         draw = gray,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
     },
%     xmin=-10.0,
%     xmax=120.0,
%     ymin=-5,
%     ymax=30.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot2,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=z, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard] {figures/figureRealworld/VINS/stamped_groundtruth.txt};

\foreach \f in {VINS,SVO_GPS, SVO_LC,ORB,SVO-MR} {
	\addplot+ [methods] table [x=x, y=z, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard ] {figures/figureRealworld/\f/stamped_traj_estimate_aligned.txt};
}

\end{axis}

\draw (legend.north -| plot1.west) rectangle (legend.south -| plot2.east);

\end{tikzpicture}

==> figures/figureSimulation/figure_simulation.tex <==
%!TEX root = ../Plots.tex

\begin{tikzpicture}[>=latex]
\tikzstyle{every node}=[font=\footnotesize]

\tikzstyle{groundtruth}=[black, thick,  line join=bevel]
\tikzstyle{methods}=[thick, line join=bevel]

\begin{axis} [
	at={(0cm, 0cm)},
	width = 7.7cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {y [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 6,
     legend cell align={left},
     legend style ={
     	at = {(1.0, 1.04)},
         draw = none,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
         anchor=south,
         name=legend,
     },
     xmin=-20.0,
     xmax=120.0,
     ymin=-10.0,
     ymax=160.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot1,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=y, col sep=space, ignore chars={\#}, each nth point=20, filter discard warning=false, unbounded coords=discard] {figures/figureSimulation/VINS/stamped_groundtruth.txt};

\foreach \f in {VINS,SVO_GPS, SVO-LC,ORB,SVO-MR} {
	\addplot+ [methods] table [x=x, y=y, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard ] {figures/figureSimulation/\f/stamped_traj_estimate_aligned.txt};
}

\addlegendentry{Groundtruth};
\addlegendentry{VINS-Fusion};
\addlegendentry{SVO-GPS};
\addlegendentry{SVO-Loop Closure};
\addlegendentry{ORB-SLAM3};
\addlegendentry{SVO-Digital Twin (ours)};
\end{axis}

\begin{axis} [
	at={(8.5cm, 0cm)},
	width = 7.5cm,
	height = 4cm,
     title style = {yshift=-6pt},
     xlabel shift = -3pt,
     ylabel shift = -5pt,
     xlabel = {x [m]},
     ylabel = {z [m]},
     cycle list={{matlab1},{matlab2},{matlab3},{matlab4},{matlab5},{matlab6},{matlab7},{matlab8}},
     legend columns = 1,
     legend cell align={left},
     legend style ={
         draw = gray,
         fill opacity=0.8,
         text opacity=1.0,
         draw opacity=1.0,
     },
     xmin=-10.0,
     xmax=120.0,
     ymin=-5,
     ymax=30.0,
%     axis equal image,
     xmajorgrids,
     ymajorgrids,
     name = plot2,
     scale only axis,
]

\addplot+ [groundtruth] table [x=x, y=z, col sep=space, ignore chars={\#}, each nth point=20, filter discard warning=false, unbounded coords=discard] {figures/figureSimulation/VINS/stamped_groundtruth.txt};

\foreach \f in {VINS,SVO_GPS, SVO-LC,ORB,SVO-MR} {
	\addplot+ [methods] table [x=x, y=z, col sep=space, ignore chars={\#}, each nth point=30, filter discard warning=false, unbounded coords=discard ] {figures/figureSimulation/\f/stamped_traj_estimate_aligned.txt};
}

\end{axis}

\draw (legend.north -| plot1.west) rectangle (legend.south -| plot2.east);

\end{tikzpicture}

==> figures/figure_1.tex <==
\tdplotsetmaincoords{25}{-20}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
\begin{tikzpicture}[tdplot_main_coords,
    >=stealth, line cap=round, line join=round,
    lines/.style={gray!50, thick}, 
    axis/.style={black, thick},
    plate/.style={},
    markers/.style={orange, thick},
    scale=1.0]
\tikzset{RPY/.style={x={(\nxx,\nxy)},y={(\nyx,\nyy)},z={(\nzx,\nzy)}}}

%\draw [draw=none] (-8.3cm,-8.3cm) rectangle (8.3cm,8cm);

%%%%%%%%%%%%%%%%%%%%% BUILDING %%%%%%%%%%%%%%%%%%%%%%

\def\w{6.5}
\def\d{3.5}
\def\h{7}
\def\mapspt{0.05cm}

\def\laserrange{3}

\def\cubeyaw{0}
\rotateRPY{0}{0}{\cubeyaw}

\begin{scope}[shift={(0, 0, 0)}, RPY]
\coordinate (f1) at (0,0,\h) ;
\coordinate (f2) at (0,0,0) ;
\coordinate (f3) at (\w,0,0) ;
\coordinate (f4) at (\w,0,\h) ;
\coordinate (b1) at (0,\d,\h) ;
\coordinate (b2) at (0,\d,0) ;
\coordinate (b3) at (\w,\d,0) ;
\coordinate (b4) at (\w,\d,\h) ;

\coordinate (right_face_center) at (0, 0.5 * \d, 0.5 *\h);
\coordinate (front_face_center) at (0.5 * \w, 0, 0.5 *\h);
\coordinate (top_face_center) at (0.5 * \w, 0.5 * \d, \h);

\node [canvas is yz plane at x=0 , text width = \d cm, inner sep = 0pt, outer sep = 0pt,  opacity = 0.7] at (right_face_center) {\includegraphics[width= \d cm, height=\h cm]{figures/texture.jpg}};
\path [draw]  (b1) -- (b2) -- (f2) -- (f1) -- cycle; % left plane
%
\node [canvas is xz plane at y=0 , text width = \w cm, inner sep = 0pt, outer sep = 0pt, opacity = 0.7] at (front_face_center) {\includegraphics[width= \w cm, height=\h cm]{figures/texture.jpg}} ;
\path [draw]  (f1) -- (f2) -- (f3) -- (f4) -- cycle; % front plane

\node [canvas is xy plane at z=0, text width = \w cm, inner sep = 0pt, outer sep = 0pt, opacity=0.7] at (top_face_center)  {\includegraphics[width= \d cm, height=\w cm, angle=90]{figures/roof.jpg}};


\tikzset{mapsarea/.style={fill= green!50!white, opacity = 0.5, draw=gray, draw opacity = 1.0}}
% front wall maps points
\foreach \x [count = \nx] in {0.25,1.0,...,\w} {
	\foreach \z [count = \nz] in {0.25,1.25,...,\h} {
		\pgfmathparse{\nx-1}
		\pgfmathtruncatemacro\nxm{\pgfmathresult}		
		\pgfmathparse{\nz-1}
		\pgfmathtruncatemacro\nzm{\pgfmathresult}	
		
		\coordinate (pt_front_\nx_\nz) at (\x + 0.1 * rand, 0.05 * rand , \z + 0.1*rand) ;
		
		\ifthenelse{1 = \nx \OR 1 = \nz} {
			% pass
		} { 
			\path [mapsarea] (pt_front_\nx_\nz)  -- (pt_front_\nx_\nzm) -- (pt_front_\nxm_\nzm)  -- (pt_front_\nxm_\nz) -- cycle ;
		}
		
		\shade [ball color = green] (pt_front_\nx_\nz) circle (\mapspt);
	}
}

% side wall maps points
\foreach \y [count = \ny] in {0.5,1.5,...,\d} {
	\foreach \z [count = \nz] in {0.25,1.25,...,\h} {
		\pgfmathparse{\ny-1}
		\pgfmathtruncatemacro\nym{\pgfmathresult}		
		\pgfmathparse{\nz-1}
		\pgfmathtruncatemacro\nzm{\pgfmathresult}	
		
		\coordinate (pt_left_\ny_\nz) at  (0.05 * rand, \y + 0.1 * rand, \z + 0.1 * rand);
		
		\ifthenelse{1 = \ny \OR 1 = \nz} {
 			\ifthenelse{\NOT 1 = \nz} {
 				\path [mapsarea] (pt_left_\ny_\nz)  -- (pt_left_\ny_\nzm) -- (pt_front_1_\nzm)  -- (pt_front_1_\nz) -- cycle ;
 			} {
 				% Pass (lower border)
 			}
		} { 
			\path [mapsarea]  (pt_left_\ny_\nz)  -- (pt_left_\ny_\nzm) -- (pt_left_\nym_\nzm)  -- (pt_left_\nym_\nz) -- cycle ;
		}
		
		\shade [ball color = green] (pt_left_\ny_\nz) circle (\mapspt);
	}
}

\end{scope}

\node (text_maps) [green!75!black, text width = 4cm, align=center, fill=white, fill opacity = 0.8, text opacity = 1.0] at (3,3,3) {\footnotesize Pointcloud from Google Maps \\[-4pt](no image data)};
\path (pt_front_4_6) -- coordinate [midway] (arrow_target) (pt_front_5_7);
\draw [->,green!50!white, thick] (text_maps.south) to [out = -45, in=-10] (arrow_target);


%%%%%%%%%%%%%%%%%%%%% DRONES %%%%%%%%%%%%%%%%%%%%%%
\def\l{0.5}
\def\r{0.32}
\def\f{1.2}
\def\imgw{1.5}
\def\imgh{2}
\def\viopt{0.04cm}

\readlist\featx{1,1.2,0,1.8};
\readlist\featy{-2.4, -2.6, -2.4,-2.4};
\readlist\featz{2.5, 5.0, 4.5,2.7};

\readlist\dronex{-2, 0.85, 3.5}
\readlist\droney{-5, -5.5, -4}
\readlist\dronez{4.62, 4.62, 4.62}

\foreach \i in {1,...,3} {
	\coordinate (drone_t\i) at (\dronex[\i], \droney[\i], \dronez[\i]);
}

\edef\nfeat{\listlen\featx[]}
\foreach \i in {1,...,\nfeat} {
	\coordinate (feat_\i) at (\featx[\i], \featy[\i], \featz[\i]);
}

\coordinate (drone_start) at (4, -4, -2);

\draw [densely dotted, gray] (drone_start) -- (drone_t3) -- (drone_t2) -- (drone_t1);

\tikzset{imageplane/.style={canvas is yz plane at x=\f , text width =  \imgw cm, inner sep = 0.2pt, outer sep = 0pt, draw=frustrumcolor, thick,  text opacity=0.8, draw opacity = 1}}
\colorlet{frustrumcolor}{black!40!white}


						%%%% DRONE 1 %%%%
\def\droneyaw{60}
\rotateRPY{0}{0}{\droneyaw}
\begin{scope}[shift={(drone_t1)}, RPY]
\colorlet{dronecolor}{red!20!white}
%\colorlet{frustrumcolor}{black!100!white}

\begin{pgfonlayer}{background}
\draw [ultra thick, dronecolor] (-\l, -\l, 0) [fill=dronecolor] circle (\r)  -- (\l, \l, 0) [fill] circle (\r);
\draw [ultra thick, dronecolor] (-\l, \l, 0)  [fill=dronecolor] circle (\r) -- (\l, -\l, 0)  [fill] circle (\r);
\end{pgfonlayer}

\node [imageplane] at (drone_t1) {\includegraphics[width=\imgw cm, height=\imgh cm]{figures/test-19.jpg}} ;
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw, -0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw,-0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw, 0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw,0.5*\imgh);
\node [below, fill = white, fill opacity = 0.75, text opacity = 1.0, inner sep = 1pt, outer sep =  1pt] {\scriptsize $t=t_{k}$};
%\path [draw]  (f1) -- (f2) -- (f3) -- (f4) -- cycle; % front plane

\end{scope}

						%%%% DRONE 2 %%%%
\def\droneyaw{100}
\rotateRPY{0}{0}{\droneyaw}
\begin{scope}[shift={(drone_t2)}, RPY]
\colorlet{dronecolor}{red!10!white}
%\colorlet{frustrumcolor}{black!70!white}

\begin{pgfonlayer}{background}
\draw [ultra thick, dronecolor] (-\l, -\l, 0) [fill=dronecolor] circle (\r)  -- (\l, \l, 0) [fill] circle (\r);
\draw [ultra thick, dronecolor] (-\l, \l, 0)  [fill=dronecolor] circle (\r) -- (\l, -\l, 0)  [fill] circle (\r);
\end{pgfonlayer}

\node [imageplane] at (drone_t2) {\includegraphics[width=\imgw cm, height=\imgh cm]{figures/test-19.jpg}} ;
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw, -0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw,-0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw, 0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw,0.5*\imgh);
\node [below, fill = white, fill opacity = 0.75, text opacity = 1.0, inner sep = 1pt, outer sep =  1pt]   {\scriptsize $t=t_{k-1}$};
\end{scope}

						%%%% DRONE 3 %%%%
\def\droneyaw{150}
\rotateRPY{0}{0}{\droneyaw}
\begin{scope}[shift={(drone_t3)}, RPY]
\colorlet{dronecolor}{red!5!white}
\begin{pgfonlayer}{background}
\draw [ultra thick, dronecolor] (-\l, -\l, 0) [fill=dronecolor] circle (\r)  -- (\l, \l, 0) [fill] circle (\r);
\draw [ultra thick, dronecolor] (-\l, \l, 0)  [fill=dronecolor] circle (\r) -- (\l, -\l, 0)  [fill] circle (\r);
\end{pgfonlayer}

\node [imageplane] at (drone_t3) {\includegraphics[width=\imgw cm, height=\imgh cm]{figures/test-20.jpg}} ;
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw, -0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw,-0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, 0.5*\imgw, 0.5*\imgh);
\draw [frustrumcolor] (0,0,0) -- (\f, -0.5*\imgw,0.5*\imgh);

\node [below, fill = white, fill opacity = 0.75, text opacity = 1.0, inner sep = 1pt, outer sep =  1pt]   {\scriptsize $t=t_{k-2}$};
\end{scope}

						%%%% DRONE START %%%%
\def\droneyaw{90}
\rotateRPY{0}{0}{\droneyaw}
\begin{scope}[shift={(drone_start)}, RPY]
\colorlet{dronecolor}{gray!15!white}
\colorlet{frustrumcolor}{black!40!white}
\draw [ultra thick, dronecolor] (-\l, -\l, 0) [fill=dronecolor] circle (\r)  -- (\l, \l, 0) [fill] circle (\r);
\draw [ultra thick, dronecolor] (-\l, \l, 0)  [fill=dronecolor] circle (\r) -- (\l, -\l, 0)  [fill] circle (\r);

\node [below, fill = white, fill opacity = 0.75, text opacity = 1.0, inner sep = 1pt, outer sep =  1pt]   {\scriptsize $t=0$};
\end{scope}
\node [below=0.5cm of drone_start] {\footnotesize Initialization through GPS};

%%%%%%%%%%%%%%%%%%%%% VIO MESH %%%%%%%%%%%%%%%%%%%%%%

\foreach \i in {1,...,\nfeat} {
	\node [star,  star point height=.08cm, minimum size=\viopt, draw, inner sep = 1pt, outer sep = 1pt, fill=blue, draw=blue] at (feat_\i	) {};
}

\foreach \didx in {1,...,3} {
	\foreach \fidx in {1,...,\nfeat} {
		\pgfmathparse{1.05*\f / sqrt((\featx[\fidx] - \dronex[\didx])^2 + (\featy[\fidx] - \droney[\didx])^2 + (\featz[\fidx] - \dronez[\didx])^2)};
		\pgfmathsetmacro{\factor}{\pgfmathresult};
	
		\coordinate (tmp) at ({ \factor * (\featx[\fidx] - \dronex[\didx]) + \dronex[\didx]}, { \factor * (\featy[\fidx] - \droney[\didx]) + \droney[\didx]}, { 	\factor * (\featz[\fidx] - \dronez[\didx]) + \dronez[\didx]});
		
		
		\draw [blue!50!black] (drone_t\didx) -- (tmp);
		\begin{pgfonlayer}{background}
			\draw [blue!50!black] (tmp) -- (feat_\fidx);
		\end{pgfonlayer}
	}
}

\tikzset{vioarea/.style={ opacity = 0.35, draw opacity = 1.0, draw=none}}
\draw [vioarea] (feat_1) -- (feat_4) -- (feat_2) -- (feat_3) -- cycle;

\node [blue] at (-1.5, -2.3, 4) (viotext) {\footnotesize VIO Features};
\draw [blue!50!black, ->] (viotext) to [out = 60, in = 210] ([shift={(-0.15,0,0)}]feat_3);
\draw [blue!50!black, ->] (viotext) to [out = 30, in = 210] ([shift={(-0.15,0,0)}]feat_1);

\path (pt_front_2_2) -- coordinate [midway] (mesh_center_1) (pt_front_3_3);
\path (pt_front_2_4) -- coordinate [midway] (mesh_center_2) (pt_front_3_5);
\path (pt_front_1_4) -- coordinate [midway] (mesh_center_3) (pt_front_2_5);
\path (pt_front_3_3) -- coordinate [midway] (mesh_center_4) (pt_front_4_4);

%\tikzset{nicearrow/.style={out = 135, in = -45}}
\tikzset{nicearrow/.style={}}
\colorlet{aligncolor}{red!80!black}
\draw [<->, thick, aligncolor] ([shift={(0,0.15,0)}]feat_1) to [nicearrow]  (mesh_center_1);
\draw [<->, thick, aligncolor] ([shift={(0,0.15,0)}]feat_2) to [nicearrow]  (mesh_center_2);
\draw [<->, thick, aligncolor] ([shift={(0,0.15,0)}]feat_3) to [nicearrow]   node [aligncolor, midway, left=1mm , fill=white, fill opacity = 0.85, text opacity = 1.0, inner sep = 2pt] {\footnotesize Alignment} (mesh_center_3);
\draw [<->, thick, aligncolor] ([shift={(0,0.15,0)}]feat_4) to [nicearrow]  (mesh_center_4);
\end{tikzpicture}

==> figures/oerlikon_pc_roxane.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/Results/oerlikon_prebuild_map.png}  % Adjust the width as needed
    \caption{Point Cloud of Zurich extracted from Google 3D tiles}
    \label{fig:zurich_pc}
\end{figure}

==> figures/sim_trans_err_roxane.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Results/error_over_time (3).pdf}  % Adjust the width as needed
    \caption{Simulation Results : Translationnal error over time}
    \label{fig:transerrorovertime}
\end{figure}

==> figures/sim_xy_view_roxane.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Results/Flightmare_trajectory_top (2).pdf}  % Adjust the width as needed
    \caption{Simulation Results : X-Y trajectory}
    \label{fig:xytraj}
\end{figure}

==> figures/sim_xz_view_roxane.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Results/Flightmare_trajectory_side (2).pdf}  % Adjust the width as needed
    \caption{Simulation Results : X-Z trajectory}
    \label{fig:xztraj}
\end{figure}

==> figures/test.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/test.png}
    % \vspace*{-12pt}
    \caption{Test figure.}
    % \vspace*{-9pt}
    \label{fig:test}
\end{figure}

==> sections/methodology_v1.tex <==
\section{Methodology}\label{sec:Related_work}

\subsection{Notation}

\begin{figure}[h]
   \centering
   \includegraphics[]{images/Methodology/CoordinateFrames.png}
   \caption{Reference frames used in this work}
   \label{img:methodology_ref_frames}
\end{figure}

The main coordinates frames are illustrated in Fig. \ref{img:methodology_ref_frames}. The primary coordinate frames used in our approach are illustrated in Fig. \ref{img:methodology_ref_frames}. For simplicity, we assume that the GPS measurements, typically received in the geodetic coordinate system (latitude, longitude, altitude), have already been transformed into an East-North-Up (ENU) frame. This ENU frame is locally linearized around an arbitrary point, which we designate as the origin of our world frame, denoted as $W$. The $W$ frame is aligned with gravity, and all subsequent measurements will be expressed in this Cartesian coordinate system (x, y, z) rather than in geodetic coordinates.

% Our problem is formulated as a sliding window optimization, with XXX.
% \begin{itemize}
%     \item \textbf{ECEF Frame}: Earth-Centered, Earth-Fixed (ECEF) frame. A global reference frame that rotates with the Earth, with its origin at the center of the Earth.
%     \item \textbf{Geodetic Frame}: Latitude, Longitude, Altitude Frame. Typically, GPS measurements are expressed in this frame
%     \item \textbf{World Frame}: Set as the ENU (East-North-Up) frame, a linearized version of the geocentric frame centered around the initial GPS measurement. This frame is aligned with gravity. GPS measurements are automatically converted to this frame upon receipt, and, for simplicity of notation, we will omit the transformation geodetic to world frame in the following chapters. The known map is also represented in this frame.
%     \item \textbf{Local Frame}: Used for our optimizations and also aligned with gravity. The origin is set at the starting point of our VIO system. It is related to the World frame via a 3D translation and a yaw rotation.
%     \item \textbf{Body Frame}: Also the IMU frame, fixed to our moving UAV
%     \item \textbf{Camera Frame}: Oriented with z pointing forward along the camera axis and y pointing downward. Features are primarily detected in this frame, producing bearing vectors from the camera's optical center to the 3D points. Calibration of the translation from this frame to the Body frame is required before initiating the algorithm.    
% \end{itemize}

\subsection{Problem formulation}

We based our work on SVO-GPS \cite{cioffi2020tightly}, a moving window state estimation framework that tightly fuses a monocular camera, an IMU, and optionally GPS. This translates to minimizing the following equation:

\begin{equation} \label{Eq:VIO_Formulation}
\begin{split}
    \min_{\mathcal{X}} \mathcal{J} = \min_{\mathcal{X}} & \sum_{k=0}^{K-1} \sum_{j\in\mathcal{L}} \left\| \mathbf{e}_v^{j,k} \right\|^2_{W_v^{j,k}} 
    + \sum_{k=0}^{K-1} \left\| \mathbf{e}_i^{k} \right\|^2_{W_i^k} \\
    &+ \sum_{k=0}^{K-1} \sum_{j\in\mathcal{G}_k} \left\| \mathbf{e}_g^{j,k} \right\|^2_{W_g^{k}}
    + \left\| \mathbf{e}_p \right\|^2  
\end{split}
\end{equation}

with: 

\begin{itemize}
\item $K$: Total number of time steps.
\item $\mathcal{L}$: Set of features.
\item $\mathbf{e}_v^{j,k}$: Reprojection error of feature $j$ at time step $k$, more precisely, $\mathbf{e}_v^{j,k} = \mathbf{z}^{j,k} - h(\mathbf{l}^w_j)$.
\item $W_l^{j,k}$: Weighting matrix for residual $j$ of type $l$ at time step $k$
\item $\mathbf{e}_i^{k}$: Inertial error vector at time step $k$.
\item $\mathbf{e}_g^{j,k}$: Global position  residual at time k for measurement j
\item $\mathbf{e}_p$: Marginalization error vector (refer to \cite{Leutenegger} for more details).
\end{itemize}

We aim to add new global measurements based on the geometry of the environment. 

\subsection{Pose constraint derivation}

After initializing our system, we always keep track of it in both the local and global frames. This allows us to use local registration techniques between our locally optimized landmarks and the global model of the surroundings, using our position in the world frame as a prior.

The Iterative Closest Point (ICP) point-to-plane algorithm was chosen, as it has the advantages of observability derivation and light-weightedness. As a reminder, ICP point-to-plane minimizes the function:

\begin{equation} \label{eq:min_ICP_function_p2plane}
\min_{\bm{\delta R}, \boldsymbol{\delta p}} f_{pn}(\bm{\delta R}, \boldsymbol{\delta p}) = \sum_{i=1}^{N} \left( \left[ \bm{\delta R} a_i + \bm{\delta p} - b_i \right] \cdot \bm{n}_i \right)^2
\end{equation}

with :

\begin{itemize}
    \item \(\bm{\delta R,p}\) : Transformation aligning the source point cloud to the target point cloud. 
    \item \(a_i\) : \(i\)th point in the source point cloud.
    \item \(b_i\) : Closest corresponding point in the target point cloud
    \item \(\bm{n}_i\) : Normal vector at the point \(b_i\) on the target point cloud    
    \item \(N\) : Total number of point pairs
\end{itemize}

In our case, the source point cloud refers to the ensemble of landmarks being optimized by the Visual-Inertial Odometry (VIO) system, while the target point cloud is created from the 3D model of the city.

% In our case, the target point cloud is created from the 3D model of the city, and the source point cloud is the ensemble of landmarks being optimized by the VIO system.

An important assumption is that we assume the bearing vectors, that the unit vectors that defines the direction from the camera to a 3D landmark, are consistent. The difference between the 3D computed landmarks and the world map comes from the drift of the body frame. Mathematically, this means: $\mathbf{\hat{p}_i} = \mathbf{p_i}$. 

Let us define $\textbf{T}^k_R = [\bm{\delta R} | \bm{\delta p}]$ as the solution of Eq. \ref{eq:min_ICP_function_p2plane} at time $k$, that is the transformation matrix that aligns the local generated point cloud to the city map. We can then derive : 


\begin{align}    
    \mathbf{T}^k_{\text{R}} \cdot {a_i} &= {b_i} + \epsilon \\
    \mathbf{T}^k_{\text{R}} \cdot \hat{\mathbf{T}}^k_{\text{WB}} \cdot  \mathbf{T}_{BC} \cdot \hat{p_i} &= \mathbf{T}^k_{WB} \cdot \mathbf{T}_{BC} \cdot {p_i} + \epsilon \\
    % \mathbf{T}^{i}_{\text{R}} \cdot \hat{\mathbf{T}}^{i}_{\text{WB}}  &= \mathbf{T}^{i}_{WB} + \epsilon \\
    \mathbf{T}_{LW} \cdot \mathbf{T}^k_{\text{R}} \cdot \hat{\mathbf{T}^k}_{\text{WB}} \cdot \hat{\mathbf{T}}_{\text{LW}}  &= \mathbf{T}^k_{LB}  + \epsilon 
\end{align}

$\mathbf{T}_{LW} \cdot \mathbf{T}^k_{\text{R}} \cdot \hat{\mathbf{T}}^{i}_{\text{WB}} \cdot \hat{\mathbf{T}}_{\text{LW}}$ is the global pose measurement that we will add to our graph. From now on we define : 
\begin{equation} \label{eq:PoseDerivationCalculation}
    \mathbf{T}^k_{M} = \mathbf{T}_{LW} \cdot \mathbf{T}^{k}_{\text{R}} \cdot \mathbf{T}_{WL}
\end{equation}

\subsection{Adaptive weighting}

The registration of two-point clouds does not necessarily yield a unique solution. 3D structures, such as corridors or circular rooms, can lead to unobservable directions. In urban environments, we often encounter many planes and collinear or coplanar points, such as streets and building facades. These scenarios may render certain directions unobservable. It is important for our system to properly manage ICP constraints; an unobservable direction should not prevent the ICP algorithm from constraining the system in other observable directions. To this end, we implement a dynamic weighting strategy based on the covariance of the ICP point-to-plane. We based ourselves out of the derivation from Barczyk et al. \cite{Barczyk_ICP}
to compute the covariance at the linearization point.

Mathematicly, Eq \ref{eq:min_ICP_function_p2plane} can be rewritten at the linearization point as 
\begin{equation}
f(x) = \sum_{i} \left|\left| \bm{y_i} - \bm{A_i} \bm{x} \right|\right|^2
\end{equation}

where:
\begin{equation}
\textbf{y}_i = \textbf{n}_i^T (\textbf{a}_i - \textbf{b}_i), \quad \textbf{A}_i = \begin{bmatrix} -(\textbf{a}_i \times \textbf{n}_i)^T \ -\textbf{n}_i^T \end{bmatrix}
\end{equation}

The covariance is then equivalent to the inverse of the Hessian \( \textbf{H}_{pn} = \sum_{i} (\bm{A_i}^T \bm{A_i}) \). Finally, for robustness, our final weight matrix also accounts for fitness, the inlier RMSE score, and includes a normalization factor. 

\begin{equation}
\label{eq:weightICP}
\begin{aligned}
\textbf{W}_M^k &= \frac{1}{\sigma^2} \cdot \textbf{H}_{pn} \cdot \beta \cdot \exp\left(-\frac{\gamma^2}{2}\right) \\
% W_i^L &= \begin{cases}
% -\beta & \text{if } w_i < -\beta \\
% w_i & \text{if } -\beta \leq W_i \leq \beta \\
% \beta & \text{if } w_i > \beta 
% \end{cases}
\end{aligned}
\end{equation}

with:
\begin{itemize}
\item $\beta$ : Scaling factor,
\item $\gamma$ : Inlier RMSE,
\item $\sigma^2 = \sum_{j=1}^{n} (\textbf{H}_{pn})_{jj}$ the sum of the diagonal elements of $\textbf{H}_{pn}$.
\end{itemize} 


\subsection{Residual Derivation}

The final residual is a pose measurement, defined as:
\begin{equation}
\mathbf{e}_{m}^{k} = \begin{bmatrix}
_L\hat{\mathbf{p}}^k_{\text{LB}}- \mathbf{p}^k_{\text{M}} \\
2 \times \text{Im}(\mathbf{q}^k_{\delta})
\end{bmatrix}
\end{equation}

with: 
\begin{itemize}
    \item $\hat{\mathbf{p}}^k_{\text{LB}}$ : Estimated VIO pose of our body in world frame
    \item $\mathbf{p}^k_{\text{M}}$ and $\mathbf{q}^k_{\text{M}}$ : Derived from $\textbf{T}^k_{M}$ of eq. \ref{eq:PoseDerivationCalculation}. 
    \item \( \mathbf{q}^k_{\delta} \) : Quaternion representing the rotation error $\mathbf{q}^k_{\delta} = \mathbf{q}^k_{\text{M}} \otimes \hat{\mathbf{q}}_{\text{LB}}^{-1k}$
    
\end{itemize}

The map registration measurements are calculated in a different thread from the optimization system, and their timestamp coincides with the timestamp of the generated point cloud from the VIO and its associated pose. This removes the need for IMU integration and allows time for the registration, as it will be simply integrated into the keyframe associated with the corresponding timestamp.
They can be integrated inside of Eq \ref{eq:min_ICP_function_p2plane} as follow :

 \begin{equation} \label{eq:VIO_GPS_Formulation}
     \min_{\mathcal{X}} \mathcal{J}_{M} = 
     \min_{\mathcal{X}} \mathcal{J} + \min_{\mathcal{X}} \sum_{k=0}^{K-1}  \left\| \mathbf{e}_{m}^{k} \right\|^2_{W_M^{k}} 
 \end{equation}
with: 
\begin{itemize}
    \item $\hat{\mathbf{p}}^k_{\text{LB}}$ : Estimated VIO pose of our body in world frame
    \item $\mathbf{p}^k_{\text{M}}$ and $\mathbf{q}^k_{\text{M}}$ : Derived from $\textbf{T}^k_{M}$ of eq. \ref{eq:PoseDerivationCalculation}. 
    \item \( \mathbf{q}^k_{\delta} \) : Quaternion representing the rotation error $\mathbf{q}^k_{\delta} = \mathbf{q}^k_{\text{M}} \otimes \hat{\mathbf{q}}_{\text{LB}}^{-1k}$
    \item $\mathbf{W}^k_{\text{M}}$ : Weight derived in Eq \ref{eq:weightICP}
\end{itemize}

\subsection{Frame alignment}

We have augmented the SVO-GPS system with an initial frame alignment procedure, which involves solving the following optimization problem:

\begin{equation}  \label{eq:FrameAlignement}
\arg \min_{\textbf{R}_z, \textbf{t}} \sum_{j=0}^{N-1} \| \textbf{p}_j - \textbf{R}_z \hat{\textbf{p}}_j - \textbf{t} \|^2
\end{equation}

The closed-form solution to Eq. \ref{eq:FrameAlignement} is derived from the work of Zhang et al. \cite{Leastsquaresfitting}. This solution is recalculated as more measurements are collected over time, refining the alignment process continuously. To ensure the alignment is robust, we employ the convergence criteria proposed by Boche et al. \cite{boche2022visualinertial}, which imposes a threshold on the yaw covariance. The convergence is evaluated by calculating the Hessian of the alignment:

\begin{equation}
\label{eq:init_hessian}
    \mathbf{H} = \sum_{j=1}^{N_\mathrm{g}} \left( {\mathbf{E}_\mathrm{g}^{j}}^{T} \mathbf{W}_\mathrm{g}^{j} \mathbf{E}_\mathrm{g}^{j} \right)
\end{equation}

where:
\begin{equation}
{\mathbf{E}_\mathrm{g}^{k}}^{T} = 
\left[ -\mathbf{R}_{WL} \quad \mathbf{R}_{WL} \left[\mathbf{R}_{LB} \mathbf{p}_{P}\right]_{\times} \right],
\end{equation}

and the condition for convergence is set by ensuring that $H^{-1}[{n,n}] < \epsilon$. \

Our alignment approach differs from traditional methods by incorporating a two-step process:

\begin{itemize}
\item Initial Alignment: The trajectory calculated by our VIO framework is aligned with the trajectory provided by the GPS. This step establishes an initial estimate of the transform.
\item Refinement Alignment: Before integrating new global measurements, we apply the Umeyama technique to realign the VIO trajectory with the poses provided by our map registration algorithm, thereby refining the transform. The prior for this iterative closest point (ICP) alignment is derived from the initial alignment step.
\end{itemize}

This two-step refinement is valuable because, although GPS measurements can be noisy or biased, they tend to be smooth over time. Consequently, during the first alignment, the yaw covariance might be low even if there is a systematic offset. The refinement step addresses this by further adjusting the alignment, ensuring a more accurate and reliable result.






==> tables/realworld_alignment_error_roxane.tex <==
\begin{table}[h!]
\centering
\caption{Initial frame alignement accuracy}
\label{tab:framealignement}
\begin{tabular}{lccc}
\hline
\textbf{Framework} & \textbf{Translation error (m)} & \textbf{Yaw Error (\textdegree)}\\
\hline
GPS-only alignement & 8.1067 & 6.7703\\
Refinement & 0.4954 & 0.7851  \\
\hline
\end{tabular}
\end{table}

==> tables/realworld_atep_roxane.tex <==
\begin{table}[h!]
\centering
\caption{Real World Results: Translation Errors}
\label{tab:rw_results}
\begin{tabular}{lcccc}
\hline
\textbf{Framework} & \textbf{Mean (m)} & \textbf{RMSE (m)} & \textbf{STD (m)} & \textbf{Med (m)} \\
\hline
\textbf{MR-SVO} & \textbf{1.006} & \textbf{1.093} & \textbf{0.425} & \textbf{0.945} \\
VINS-Mono & 4.049 & 1.608 & 2.199 & 3.303 \\
SVO-GPS & 2.465 & 3.047 & 1.792 & 1.676 \\
ORB-SLAM & 1.861 & 2.360 & 1.453 & 1.312\\
SVO-Loop Closure & 1.309 & 1.603 & 0.925 & 1.115\\
MR-SVO constante weights & 1.617 & 2.115 & 1.363 & 0.98\\
\hline
\end{tabular}
\end{table}

==> tables/realworld_ater_roxane.tex <==
\begin{table}[h!]
\centering
\caption{Real World Results: Rotation Errors}
\label{tab:rw_results_rot}
\begin{tabular}{lcccc}
\hline
\textbf{Framework} & \textbf{Mean (\textdegree)} & \textbf{RMSE (\textdegree)} & \textbf{STD (\textdegree)} & \textbf{Med (\textdegree)} \\
\hline
\textbf{MR-SVO} & \textbf{2.846} & \textbf{3.395} & \textbf{0.425} & \textbf{1.852}  \\
VINS-Mono & 10.08 & 11.297 & 5.092 & 9.727 \\
SVO-GPS & 5.126 & 5.986 & 3.093 & 4.207 \\
ORB-SLAM & 5.664 & 7.0409 & 4.183 & 4.042 \\
SVO-Loop Closure  & 4.142 & 4.701 & 2.221 & 3.144 \\
MR-SVO-Ablation  & 4.763 & 5.496 & 2.741 & 4.763 \\
\hline
\end{tabular}
\end{table}

==> tables/realworld_error_overtime_roxane.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Results/error_over_time.pdf}  % Same alignement time for all of them
    \caption{Real World Results : Error over time}
    \label{fig:xytraj}
\end{figure}

==> tables/sim_atep_roxane.tex <==
\begin{table}[h!]
\centering
\caption{Simulation Results: Translation Errors}
\label{tab:simulation_results}
\begin{tabular}{lcccc}
\hline
\textbf{Framework} & \textbf{Mean (m)} & \textbf{RMSE (m)} & \textbf{STD (m)} & \textbf{Med (m)} \\
\hline
\textbf{MR-SVO} & \textbf{2.029} & \textbf{2.781} & \textbf{1.902} & \textbf{0.957} \\
VINS-Mono & 6.106 & 7.874 & 4.971 & 2.869 \\
SVO-GPS & 5.648 & 7.839 & 5.435 & 2.127 \\
ORB-SLAM & 3.426 & 4.324 & 2.638 & 2.642 \\
SVO-Loop closure & 3.127 & 4.021 & 2.528 & 1.618 \\
\hline
\end{tabular}
\end{table}

==> tables/sim_ater_roxane.tex <==
\begin{table}[h!]
\centering
\caption{Simulation Results: Rotation Errors}
\label{tab:simulation_results_rot}
\begin{tabular}{lcccc}
\hline
\textbf{Framework} & \textbf{Mean (\textdegree)} & \textbf{RMSE (\textdegree)} & \textbf{STD (\textdegree)} & \textbf{Med (\textdegree)} \\
\hline
\textbf{MR-SVO} & \textbf{0.791} & \textbf{0.886} & \textbf{0.399} & \textbf{0.702} \\
VINS-Mono & 1.303 & 1.303 & 0.540 & 1.073 \\
SVO-GPS & 1.083 & 1.218 & 0.558 & 1.449 \\
ORB-SLAM & 4.065 & 4.328 & 1.488 & 4.436 \\
SVO-Loop closure-SLAM & 0. & 4.328 & 1.488 & 4.436 \\
\hline
\end{tabular}
\end{table}

==> tables/test.tex <==
\begin{table}[t!]
\caption{
$\text{ATE}_{\text{T}}$ in meters and $\text{ATE}_{\text{R}}$ in degrees on one of the test sequences of the lemniscate and racing trajectory. In bold are the best values, and in underlined bold are the second-best values.}
\label{tab:absolute_erros}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Trajectory\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Eval. \\ metric\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Algorithm}} \\ \cline{3-7} 
 & & \textbf{OpenVINS} & \textbf{SVO} & \textbf{Gate-IO} & \textbf{TLIO} & \textbf{IMO (ours)}\\ \hline \hline 

\multirow{2}{*}{Lemniscate} & $\text{ATE}_{\text{T}}$ [m] & 16.81 & 22.73 & N.A. & \underline{\textbf{0.34}} & \textbf{0.24} \\ & $\text{ATE}_{\text{R}}$ [deg] & 114.9 & 106.6 & N.A. & \underline{\textbf{3.5}} & \textbf{3.4} \\
\hline
\multirow{2}{*}{Racing} & $\text{ATE}_{\text{T}}$ [m] & 98.20 & 47.20 & \textbf{0.48} & 1.21 & \underline{\textbf{0.56}} \\ & $\text{ATE}_{\text{R}}$ [deg] & 99.0 & 123.0 & \textbf{2.2} & 3.3 & \underline{\textbf{2.8}}\\
\hline
\end{tabular}
}
\end{table}
